How the world's collective attention is being paid to a pandemic: COVID-19 related n-gram time series for 24 languages on Twitter

In confronting the global spread of the coronavirus disease COVID-19 pandemic we must have coordinated medical, operational, and political responses. In all efforts, data is crucial. Fundamentally, and in the possible absence of a vaccine for 12 to 18 months, we need universal, well-documented testing for both the presence of the disease as well as confirmed recovery through serological tests for antibodies, and we need to track major socioeconomic indices. But we also need auxiliary data of all kinds, including data related to how populations are talking about the unfolding pandemic through news and stories. To in part help on the social media side, we curate a set of 2000 day-scale time series of 1- and 2-grams across 24 languages on Twitter that are most 'important' for April 2020 with respect to April 2019. We determine importance through our allotaxonometric instrument, rank-turbulence divergence. We make some basic observations about some of the time series, including a comparison to numbers of confirmed deaths due to COVID-19 over time. We broadly observe across all languages a peak for the language-specific word for 'virus' in January 2020 followed by a decline through February and then a surge through March and April. The world's collective attention dropped away while the virus spread out from China. We host the time series on Gitlab, updating them on a daily basis while relevant. Our main intent is for other researchers to use these time series to enhance whatever analyses that may be of use during the pandemic as well as for retrospective investigations.

==> bin/rename <==
#!/usr/bin/perl

$usage = "rename text1 text2 file [files...]

swap text1 for text2 in file names
whenever text1 is found.

swaps only the first instance.

rudimentary first version: use only for static text.
";

$pattern1 = $ARGV[0];
$pattern2 = $ARGV[1];

foreach $filename (@ARGV[2..$#ARGV]) {
    if ($filename =~ m/$pattern1/) {
	($newfilename = $filename) =~ s/$pattern1/$pattern2/g;
	print "renaming $filename as $newfilename...\n";
	`mv "$filename" "$newfilename"`;
    }
}


==> covid19-ngrams-revtex4.settings.tex <==
\newcommand{\filenamebase}{covid19-ngrams}


==> covid19-ngrams.abs.tex <==
In confronting the global spread of the coronavirus disease COVID-19 pandemic
we must have coordinated medical, operational, and political responses.
In all efforts, data is crucial.
Fundamentally, and in the possible absence of a vaccine for 12 to 18 months,
we need universal, well-documented testing for both the presence of the disease as
well as confirmed recovery through serological tests for antibodies,
and we need to track major socioeconomic indices.
But we also need auxiliary data of all kinds, including data related
to how populations are talking about the unfolding pandemic through news and stories.
To in part help on the social media side, we curate a set of 2000 day-scale time series of
$1$- and $2$-grams across 24 languages on Twitter that are most `important'
for April 2020 with respect to April 2019.
We determine importance through our allotaxonometric instrument, rank-turbulence divergence.
We make some basic observations about some of the time series, including a comparison to
numbers of confirmed deaths due to COVID-19 over time.
We broadly observe across all languages a peak for
the language-specific word for `virus' in January 2020 followed
by a decline through February and then a surge through March and April.
\textbf{The world's collective attention dropped away while the virus spread out from China.}
We host the time series on Gitlab, updating them on a daily basis while relevant.
Our main intent is for other researchers to use these time series to enhance whatever
analyses that may be of use during the pandemic as well as for retrospective investigations.

==> covid19-ngrams.acknowledgments.tex <==
The authors are grateful for 
support furnished by MassMutual and Google,
and the computational facilities provided
by the Vermont Advanced Computing Core.
Computations were performed 
on the Vermont Advanced Computing Core supported 
in part by NSF award No. OAC-1827314.
The authors appreciate discussions and correspondence with
Aaron Schwartz,
Todd DeLuca,
Nina Safavi,
and
Nicholas Danforth.


==> covid19-ngrams.author.tex <==
\author{
  \firstname{Thayer}
  \surname{Alshaabi}
}
\thanks{The first three authors contributed as a team.}
%% \email{thayer.alshaabi@uvm.edu}

\affiliation{
  Computational Story Lab,
  Vermont Complex Systems Center,
  MassMutual Center of Excellence for Complex Systems and Data Science,
  Vermont Advanced Computing Core,
  University of Vermont,
  Burlington, VT 05401.
  }
\affiliation{
  Department of Computer Science,
  University of Vermont,
  Burlington, VT 05401.
  }
  

\author{
  \firstname{Michael V.}
  \surname{Arnold}
}
\thanks{The first three authors contributed as a team.}
%% \email{michael.arnold@uvm.edu}

\affiliation{
  Computational Story Lab,
  Vermont Complex Systems Center,
  MassMutual Center of Excellence for Complex Systems and Data Science,
  Vermont Advanced Computing Core,
  University of Vermont,
  Burlington, VT 05401.
  }

\author{
  \firstname{Joshua R.}
  \surname{Minot}
}
\thanks{The first three authors contributed as a team.}
%% \email{joshua.minot@uvm.edu}


\affiliation{
  Computational Story Lab,
  Vermont Complex Systems Center,
  MassMutual Center of Excellence for Complex Systems and Data Science,
  Vermont Advanced Computing Core,
  University of Vermont,
  Burlington, VT 05401.
  }


\author{
  \firstname{Jane Lydia}
  \surname{Adams}
}

%% \email{jane.adams@uvm.edu}

\affiliation{
  Computational Story Lab,
  Vermont Complex Systems Center,
  MassMutual Center of Excellence for Complex Systems and Data Science,
  Vermont Advanced Computing Core,
  University of Vermont,
  Burlington, VT 05401.
}

\author{
  \firstname{David Rushing}
  \surname{Dewhurst}
}

%% \email{david.dewhurst@uvm.edu}

 \affiliation{
   Charles River Analytics, 
   Cambridge, MA 02138.
   }
   
\affiliation{
  Computational Story Lab,
  Vermont Complex Systems Center,
  MassMutual Center of Excellence for Complex Systems and Data Science,
  Vermont Advanced Computing Core,
  University of Vermont,
  Burlington, VT 05401.
  }


\author{
   \firstname{Andrew J.}
   \surname{Reagan}
 }
 
 \affiliation{
   MassMutual Data Science,
   Boston,
   MA 01002.
   }

\affiliation{
  Computational Story Lab,
  Vermont Complex Systems Center,
  MassMutual Center of Excellence for Complex Systems and Data Science,
  Vermont Advanced Computing Core,
  University of Vermont,
  Burlington, VT 05401.
  }

\author{
  \firstname{Roby}
  \surname{Muhamad}
  }

\affiliation{
International Class Program,
Faculty of Social and Political Sciences,
University of Indonesia,
Jakarta, Indonesia. 
}

 

\author{
  \firstname{Christopher M.}
  \surname{Danforth}
}

%% \email{chris.danforth@uvm.edu}

\affiliation{
  Computational Story Lab,
  Vermont Complex Systems Center,
  MassMutual Center of Excellence for Complex Systems and Data Science,
  Vermont Advanced Computing Core,
  University of Vermont,
  Burlington, VT 05401.
  }

\affiliation{
  Department of Mathematics and Statistics,
  University of Vermont,
  Burlington, VT 05401.
  }


\author{
  \firstname{Peter Sheridan}
  \surname{Dodds}
}

\email{Corresponding author: peter.dodds@uvm.edu}

\affiliation{
  Computational Story Lab,
  Vermont Complex Systems Center,
  MassMutual Center of Excellence for Complex Systems and Data Science,
  Vermont Advanced Computing Core,
  University of Vermont,
  Burlington, VT 05401.
  }

\affiliation{
  Department of Computer Science,
  University of Vermont,
  Burlington, VT 05401.
  }


==> covid19-ngrams.biblio.tex <==
\bibliography{\filenamebase}


==> covid19-ngrams.body.tex <==
%% to help with ordering because of Figure captions
\nocite{li2020a,kraemer2020a}
\nocite{dong2020a,xu2020a}
\nocite{cinelli2020a,chen2020a,lampos2020a}
\nocite{chen2020social-distance-and-sars-memory-impact-on-the-public-awareness-of-2019-novel-coronavirus-cvoid-19-outgbreak}


% data (SILK):
%% /users/s/t/storylab/www-root/share/data/covid19ngrams/data/rank_turbulence_divergence/april_top_2grams
%%
%% to get hold of top 20 1-grams, say, use
%% awk '{print $1}' ar_count.tsv | head -20

%% \section{Introduction}
%% \label{sec:covid19.intro}

\section{Overview}
\label{sec:covid19.overview}


Understanding how major disasters affect the wellbeing of populations both
in real time and historically is of paramount importance.
We especially need real-time measurement to enable policy makers in health systems and government
to gauge the immediate situation and evaluate scenarios,
and for researchers to model possible future trajectories of social systems.
Researchers have demonstrated how characterizing and tracking public discourse of the COVID-19 spread on social media~\cite{depoux2020pandemic,li2020characterizing,chen2020unpacking}
can support local authorities' efforts in response to the global pandemic~\cite{van2020using,block2020social}.
Recent studies have also investigated the impact of pre-existing political polarization on discussions related to COVID-19 
throughout Twitter's ecosystem~\cite{jiang2020political}, 
as well as the extent of misinformation on social media~\cite{bursztyn2020misinformation,jamieson2020relation, pennycook2020fighting}.
Our primary aim here is to generate a particular data stream that may be of
help to other researchers:
A principled set of $n$-gram time series across major languages
used on Twitter and news-relevant for April, 2020.
Our work is complementary to extant efforts to enable research
on the COVID-19 pandemic~\cite{li2020a,kraemer2020a}
by gathering and sharing epidemiological data~\cite{dong2020a,
  xu2020a,
  xu2020epidemiological,
  buckee2020aggregated,
  ienca2020responsible,
  lopez2020end,
  boing2020quantifying,
  holtz2020interdependence},
economic data, and internet and social media data~\cite{cinelli2020a,
  chen2020a,
  chen2020social-distance-and-sars-memory-impact-on-the-public-awareness-of-2019-novel-coronavirus-cvoid-19-outgbreak,
  lampos2020a,
  bento2020evidence}.

\begin{table}[tp!]
  \begin{tabular}{rlc}
    Rank & Language & Code \\
    \hline
    1 & English & en \\
    2 & Spanish & es \\
    3 & Portuguese & pt \\
    4 & Arabic & ar \\
    5 & Korean & ko \\
    6 & French & fr \\
    7 & Indonesian & id \\
    8 & Turkish & tr \\
    9 & German & de \\
    10 & Italian & it \\
    11 & Russian & ru \\
    12 & Tagalog & tl \\
  \end{tabular}
  \qquad
  \begin{tabular}{rlc}
    Rank & Language & Code \\
    \hline
    13 & Hindi & hi \\
    14 & Persian & fa \\
    15 & Urdu & ur \\
    16 & Polish & pl \\
    17 & Catalan & ca \\
    18 & Dutch & nl \\
    19 & Tamil & ta \\
    20 & Greek & el \\
    21 & Swedish & sv  \\
    22 & Serbian & sr \\
    23 & Finnish & fi \\
    24 & Ukrainian & uk \\
  \end{tabular}
  \caption{
    The 24 languages for which we provide COVID-19 related Twitter time series.
    }
  \label{tab:covid19.languages}
\end{table}

In this short piece,
we describe how we select languages and $n$-grams relevant to the
time period of the present COVID-19 pandemic;
show example time series plots for the word `virus' (and its translations), including a visual comparison with
COVID-19 confirmed case and death numbers;
and
describe the data sets, figures, and visualizations
for 24 languages that we share online.

\section{Selection of languages and $n$-grams}
\label{sec:covid19.methods}


We base our curation on our work in two of our previous papers~\cite{alshaabi2020a,dodds2020a},
and we draw from a database of approximately 10\% of all tweets from 2008/09/09 to present.
Our process of obtaining salient $n$-grams for April 2020 comprises two steps.
First,
we used the language identification and detection tool FastText-LID~\cite{joulin2016a,joulin2016b}
to evaluate all tweets in our historical archive,
finding over 100 languages~\cite{alshaabi2020a}.
Besides analyzing all tweets (AT), we also separately process what we call
organic tweets (OT): All Twitter messages which are original.
Organic tweets exclude retweets
while including all added text for quote tweets.
In doing so, we are able to carry through a measure of spreadability
for all $n$-grams.
The key threshold we use for spreading is the naive one from biological and social contagion models:
When an $n$-gram appears in more retweeted than organic material, we view it as being socially amplified.
We subsequently extracted day-scale 
Zipf distributions
for 1-, 2-, and 3-grams along with
day-scale $n$-gram time series~\cite{alshaabi2020b}.
We preserve case where applicable, do not apply any stemming.
We note that the top 10 languages on Twitter comprise 85\% of all tweets.
Here, we take 24 of the most commonly used languages
on Twitter in 2019, with the provision that we are able to parse them into $n$-grams.
For the time being, we are unable to reliably parse continuous-based script languages 
such as Japanese, Thai, and Chinese,
the 2nd, 6th, and 13th most common languages.
The selected languages comprise two thirds of the daily tweets on the platform.
We exclude all tweets not assigned a language with sufficient confidence
(an effective 4th ranked collection).
In other words, we select the predicted language with the highest confidence score.
If the confidence score of our FastText-LID model is less than 25\% for a given tweet, 
then we label that tweet as Undefined (und).
We also choose to include Ukranian (29th) over Cebuano (28th) 
due to a marginal degree of uncertainty for detecting messages written in Cebuano~\cite{alshaabi2020a}.
We list the 24 languages by overall usage frequency in Tab.~\ref{tab:covid19.languages}.


Second, we compare usage of $n$-grams in April of 2020 with April 2019
to determine which $n$-grams have become most elevated in relative usage.
We do so by using rank-turbulence divergence~\cite{dodds2020a}, an instrument
for comparing any pair of heavy-tailed size distributions of categorical data.
Other well-considered divergences will produce similar lists.
For each language, we take Zipf distributions for each day of April 2020,
and compare them with the Zipf distributions of 52 weeks earlier.
For an example, we show in
Fig.~\ref{fig:covid19.allotaxonometer9000-2019-04-30-2020-04-30-rank-div-alpha-third-it}
an allotaxonograph for Italian comparing 2019/04/30 and 2020/04/30.
The main plot displays a rotated 2D-histogram to avoid misinterpretation of causality. 
We bin $n$-grams logarithmically such that bins located near the center vertical line 
indicate $n$-grams that are used equivalently on both days, 
whereas bins on either side highlight $n$-grams that are used more often on the corresponding date. 
We use rank-turbulence divergence with the parameter $\alpha$ set to 1/3 as this provides
a reasonable fit to the lexical turbulence we observe~\cite{pechenick2017a,dodds2020a}.
Up to a normalization factor~\cite{dodds2020a}, we compute rank-turbulence divergence for each $n$-gram $\tau$ as follows:
\begin{align*}
     \delta D^{\textnormal{R}}_{\alpha, \tau} & \propto 
     \bigg| \dfrac{1}{r_{\tau, t_1}^{\alpha}} - \dfrac{1}{r_{\tau, t_2}^{\alpha}} \bigg|^{1 / (\alpha + 1)} 
     = 
     \bigg| \dfrac{1}{r_{\tau, t_1}^{1/3}} - \dfrac{1}{r_{\tau, t_2}^{1/3}} \bigg|^{3/4},
\end{align*}
where $r_{\tau, t_1}$ and $r_{\tau, t_2}$
indicate the rank of usage for $\tau$ at time step $t_1$ and $t_2$ respectively. 
We plot contour lines to demonstrate the scale of rank-turbulence divergence
and use divergence contributions of each $n$-gram 
to compile an ordered set of relevant $n$-grams for each day (see right panel of Fig.~\ref{fig:covid19.allotaxonometer9000-2019-04-30-2020-04-30-rank-div-alpha-third-it}).  
For ease of plotting, we have further chosen to compare the subset of words containing Latin characters only.
Words associated with the pandemic dominate the contributions from 2020/04/30.
On the right side of the allotaxonograph,
we see
`Coronavirus', 
`virus',
`quarantina',
`pandemia',
`Bergamo',
and
`morti'.
We repeat this process for every day in April, 
and combine divergence contributions for all $n$-grams across
these days, and rank $n$-grams in descending order indicating 
the most narratively dominate $n$-grams for the month of April. 



\begin{figure*}[tp!]
  \includegraphics[width=1.1\textwidth]{figures/local/figallotaxonometer9000-2019-04-30-2020-04-30-rank-div-alpha-third-it_noname.pdf}
  \caption{
    Allotaxonograph using rank-turbulence divergence for
    Italian word usage on April 30, 2019 versus April 30, 2020.
    For this visualization, we consider the subset of 1-grams that are formed from latin characters.
    The right hand sides of the rank-rank histogram and the rank-turbulence contribution list
    are dominated by COVID-19 related terms.
    See Dodds~\etal~\cite{dodds2020a} for a full explanation of our allotaxonometric instrument.
  }
  \label{fig:covid19.allotaxonometer9000-2019-04-30-2020-04-30-rank-div-alpha-third-it}
\end{figure*}
 
  
\begin{table*}[tp!]
  \includegraphics[width=.95\textwidth]{figures/local/tables/top20-1grams-tab1.png}\\
  \includegraphics[width=.95\textwidth]{figures/local/tables/top20-1grams-tab2.png}
  \caption{
    Top 20 (of 1,000) 1-grams for our top 12 languages
    for the first three weeks of April 2020 relative to a year earlier.
    Our intent is to capture 1-grams that are topically and culturally important
    during the COVID-19 pandemic.
    While overall, we see pandemic-related words dominate the lists across languages,
    we also find considerable specific variation.
    Words for virus, quarantine, protective equipment, and testing show different orderings
    (note that we do not employ stemming).
    Unrelated 1-grams but important to the time of April 2020 are in evidence; the balance
    of these are important for our understanding of how much the pandemic is being talked about.
    To generate these lists we use the allotaxonometric method of
    rank-turbulence divergence to find the most distinguishing 1-grams
    (see Sec.~\ref{sec:covid19.methods},
    Fig.~\ref{fig:covid19.allotaxonometer9000-2019-04-30-2020-04-30-rank-div-alpha-third-it},
    and Dodds~\etal~\cite{dodds2020a}).
    We note that these tables are images and cannot be copied;
    see the Sec.~\ref{sec:covid19.data} for data download sites.
  }
  \label{fig:covid19.top1grams-1}
\end{table*}

\begin{table*}[tp!]
  \includegraphics[width=.95\textwidth]{figures/local/tables/top20-1grams-tab3.png}\\
  \includegraphics[width=.95\textwidth]{figures/local/tables/top20-1grams-tab4.png}
  \caption{
    Continuing on from Fig.~\ref{fig:covid19.top1grams-1}:
    Top 20 1-grams for the second 12 of 24 languages we study
    for April 2020 relative to April 2019.
  }
  \label{fig:covid19.top1grams-2}
\end{table*} 

 
\section{Data, Visualizations, and Sites}
\label{sec:covid19.data}

For each language, and for each of the top 
$n$-grams we have identified, we extract
three day-scale time series starting on 2019/09/01:
Daily counts, 
ranks, 
and normalized frequencies based on the Eastern Time Zone (ET).
Understandably, as the pandemic was unfolding in early 2020, most regional health organizations 
could not confirm the roots or exact initial date of the first COVID-19 case within their population of charge, with speculations that the virus may have started spreading in late 2019. 
Therefore, we started our data collection on September of 2019  
to cover the last quarter of 2019 and the few months leading to the pandemic spreading worldwide. 

The degree to which the pandemic is being discussed on Twitter is
of great interest in itself, and our data set will allow for such
examination.

For the $n$-grams our method surfaces, 
we observe variations in punctuation and grammatical structures.
These variants as well as 
non-pandemic-related elements may be filtered out for individual languages by hand as may suit interested researchers.
We provide a cleaned version of the data set whereby we omit links, handles, hashtags, emojis, and punctuation. 
We also note that our decision to respect capitalization leads to $n$-grams that some researchers may wish to collapse,
and we also provide a case-insensitive version of our data set. 
We repeat all of the above steps for $n$-grams derived from organic tweets (OT).

We share and maintain all data on Gitlab at: \href{https://gitlab.com/compstorylab/covid19ngrams}{https://gitlab.com/compstorylab/covid19ngrams}.
We also provide a connected website associated with our paper at:
\href{http://compstorylab.org/covid19ngrams/}{http://compstorylab.org/covid19ngrams/}.
We show tables of the leading $n$-grams in our data set,
as well as example "bar chart races" for the dominant COVID-19 $n$-grams
in major languages.
Our intention is to automatically update the data set on Gitlab,
as soon as we have processed all tweets for a day.


We show the resulting top 20 April-2020-specific 1-grams for the 24 languages
in
Tabs.~\ref{fig:covid19.top1grams-1}
and~\ref{fig:covid19.top1grams-2}.
For display, we use the cleaned version, 
omitting hashtags, handles, emojis, numbers, and punctuation.
We also removed all variations of `Bomboclaat' from Dutch.
Overall, we see that the lists are dominated by language specific words 
for
coronavirus
virus,
quarantine,
pandemic,
testing,
and spreading.

In the full, unfiltered data set, some 1-grams such as punctuation represent functional changes in the use of Twitter across languages.
The white heart emoji
makes the top 20 in a few languages such as English, Arabic, Korean and German.
By contrast, and according to the measurements we have used here,
the worried face emoji,
\includegraphics[height=1em]{figures/local/emojis/face-with-pleading-eyes_1f97a.pdf},
%% {\NotoEmoji\symbol{"1F97A}},
has become important across many languages in April 2020 relative to April 2019.
It would be natural to see this emoji as being pandemic-related
but in fact, we see from time series that the worried emoji has slowly being increasing
in usage over time for several years
(determining the reasons for which we will leave for a separate line of inquiry).
All 1-grams are included in the shared raw version of the data sets.

We emphasize that with our approach, we do not explicitly
determine whether or not an $n$-gram is relevant
to COVID-19.
While the pandemic was one of the top stories of 2020 
for the majority of countries,
there have of course been other major events and
moments in popular culture around the world.
For example, in March 2020 for the United States, the democratic primary
leads to the 1-gram in English Twitter of `Biden' being prominent.
Similarly, we see many $n$-grams related to the
Big Brother Brazil show in Portuguese, and K-pop in Korean.
Further, most languages have a strong degree of geographic specificity
(e.g., Finnish for Finland, Portuguese for Brazil),
and we have not
filtered for precise geo-location.
English, Spanish, Arabic, and French are some of the more
geographically distributed languages.



\section{Example time series}
\label{sec:covid19.timeseries}

%% Figures: silk:www-root/share/data/covid19ngrams/plots 

\begin{figure*}[tp!]
  \includegraphics[width=\textwidth]{figures/local/silk/contagiograms_virus_12.pdf}
    \caption{
      Contagiograms for the word
      `virus' in the top 12 of the 24 languages we study here.
      \textbf{The major observation is that the world's attention peaked early in late January around the news
      of an outbreak of a new infectious disease in Wuhan,
      declining through well into February before waking back up.}
      The main plots in each panel show usage ranks at the day scale (ET).
      The solid lines indicating smoothing with a one week average (centered).
      The plots along the top of each panel show the relative fractions of each 1-gram's daily counts
      indicating as to whether they appear in retweets (RT, spreading) or organic tweets (OT, new material).
      The background shading shows when the balance favors spreading---story contagion.
      See Fig.~\ref{fig:covid19.virus2_ranks} for the next 12 languages, as well as
      Sec.~\ref{sec:covid19.timeseries} for general discussion, and Alshaabi~\etal~\cite{alshaabi2020b} for technical details of contagiograms.
    }
    \label{fig:covid19.virus1_ranks}
\end{figure*}

\begin{figure*}[tp!]
    \includegraphics[width=\textwidth]{figures/local/silk/contagiograms_virus_24.pdf}
    \caption{
      Following on from Fig.~\ref{fig:covid19.virus1_ranks},
      contagiograms for the word
      `virus' in the second 12 of the 24 languages.
      We note that some of these 1-grams are socially amplified over time,
      while others often shared organically. 
    }
    \label{fig:covid19.virus2_ranks}
\end{figure*}

 
\begin{figure*}[tp!]
    \includegraphics[width=\textwidth]{figures/local/silk/coronagrams_cases.pdf}
    \caption{
      Time series for daily reported case loads and death 
      compared with a list of 10 salient 1-grams
      for the top language spoken in each country.
      For each $n$-gram, 
      we display a weekly rolling average of usage ranks at the day scale in gray
      overlaid by an average of all these 1-grams in black 
      marking their corresponding ranks using the left vertical axis.
      Similarly, we use the right vertical axis to
      display a weekly rolling average of daily new cases (red solid-line),
      and reported new deaths (orange dashed-line).
      We note that the reported counts are underestimates, more so for cases than
      deaths, and errors are unknown.  
      We sourced data for confirmed
      cases and fatalities from Johns Hopkins University Center for
      Systems Science and Engineering's COVID-19
      project~\cite{dong2020a}.
      Starting on 2020/01/22,
      the project's data has been collected from national and regional health
      authorities across the world. The data is augmented by case
      reports from medical associations and social media posts---these
      later sources are validated against official records before
      publication.
      For the present piece, we use daily summary files for case
      counts and fatalities, although an API and online dashboard are
      available for more up-to-date reports.
    }
    \label{fig:covid19.coronagrams_cases}
\end{figure*}



We briefly consider two sets of
sample time series based on our data set.
Across Figs.~\ref{fig:covid19.virus1_ranks} and~\ref{fig:covid19.virus2_ranks},
we plot contagiograms~\cite{alshaabi2020b} 
for the word `virus' translated as appropriate
in to each of the 24 languages.
For each language, we display the daily (Zipfian) rank for `virus' in the main panel of each plot.
We add a grey background indicating the best and worst rank of each week overlaid by a centered weekly rolling average (black).
The pale disk highlights the date of maximum observed rate.
In the secondary time series at the top of each panel,
we show the relative fraction
of 1-gram contained in retweets (RT) versus organic tweets (OT).
When the RT/OT balance exceeds 50\%, we shade the background to indicate
that the 1-gram is being spread (e.g., retweeted) more than organically tweeted.
For each contagiogram, 
we also display a heatmap of the relative amplification of each 1-gram compared to the 
fraction of 1-grams that are found in RTs on that day. 
For each day of the week, 
shades of red indicate higher social amplification,
whereas gray shows that the volume of that 1-gram is often shared organically. 
See Alshaabi~\etal~\cite{alshaabi2020b} for technical details of contagiograms, 
more examples of contagiograms can also be found in Figs.~\ref{fig:covid19.1grams_samples}, and \ref{fig:covid19.2grams_samples}.

\textbf{
Alone, the highest ranks for `virus' show the enormity of the pandemic.
While a common enough word in normal times, `virus' has reached into
the top 100 ranks across many languages, a region that we have elsewhere
referred to as the realm of lexical ultrafame~\cite{dodds2019a}.
Normally only the most basic function words of a language will
populate the top 100 ranks.
}
In the last few months,
we have seen `virus' rise as high
as $r$=24 in Indonesian (2020/01/26),
$r$=27 in Polish (2020/03/11),
$r$=29 in Urdu (2020/03/22),
$r$=44 in German (2020/03/14),
and
$r$=83 in English (2020/03/13).
In terms of the shapes of the time series for `virus',
most languages show a late January peak consistent with the news from China
of a novel coronavirus disease spreading in Wuhan.
The subsequent drop in usage rate across most of the 24 languages reflects a
global decline in attention being paid to the outbreak.
The Italian time series for `virus' in
Fig.~\ref{fig:covid19.virus1_ranks}J shows an abrupt jump about
three quarters of the way through February,
strikingly just after a drop in RT/OT balance.
Persian has a similar shock jump just after
midway of February 
(Fig.~\ref{fig:covid19.virus1_ranks}B).
We see in Fig~\ref{fig:covid19.virus2_ranks}E
that `virus' in Catalan shows no early January peak
like most of the other 23 languages, suggesting that even the initial news from China
did not have great impact.

One of the major problems we face with the COVID-19 pandemic
is the unevenness of testing across the world.
South Korea and Iceland have tested early and extensively
while the United States's testing has been uncoordinated and slow to expand.
Urdu's heightened time series for `virus' (Fig~\ref{fig:covid19.virus2_ranks}C)
would seem especially concerning given low numbers coming out of Pakistan
which, as of 2020/03/24, had reported 1,063 cases and 8 deaths~\cite{dong2020a}.
For Indonesia, where testing has also been limited~\cite{dong2020a}
and with peak attention on Twitter coming in January and early focus
on economic issues and evacuation of nationals from Wuhan, a dip in
the rank of `virus' in the second half of February is also worrying (Fig~\ref{fig:covid19.virus1_ranks}G).

Countries around the world have adopted different strategies and policies in response to the coronavirus pandemic.  
While most languages have COVID-19 related terms across the top $n$-grams, 
some languages also have terms related to other big events happening simultaneously.
For example, we see many $n$-grams discussing the democratic primary election in the US. 
We also find $n$-grams connected to the Big Brother Brazil show in Portuguese,
while Korean has many K-pop references. 
This in part shows that the collective attention of different populations will, indeed, vary  
depending on the spread of the virus across countries all over the globe for the time period considered in this study. 
We note, however, 
that $n$-grams related to the pandemic can still be found in Portuguese  
showing the initial response to the news about the COVID-19 outbreak
as the virus started slowly spreading in Brazil. 

As one very simple example of comparing our Twitter times series
with pandemic-related data, in Fig.~\ref{fig:covid19.coronagrams_cases},
we present plots of daily reported cases and deaths over time
for 12 countries, along with
time series for 10 salient 1-grams in the top spoken language for each country.
We note that the reported number of cases and deaths
are subject to under-reportings.
For each country, 
we use the left vertical axis to plot 
a weekly rolling average of usage ranks at the day scale for 10 1-grams (gray lines)
translated in the top spoken language for each country,
while the black solid line shows an average of all these 1-grams.
We selected 10 1-grams from the top of each list that are directly related to the coronavirus pandemic to highlight the collective attention around the COVID-19 outbreak. 
The set of 1-grams we use for each language can be found online at:
\href{https://gitlab.com/compstorylab/covid19ngrams/-/blob/master/src/consts.py}{https://gitlab.com/compstorylab/covid19ngrams/-/blob/master/src/consts.py}.
Using the right vertical axis,
we display a weekly rolling average of daily new cases (red solid-line),
and reported new deaths (orange dashed-line).

We see a global surge of attention on Twitter starting mid March through April following the state-wide lockdowns in most countries.
Some languages such as Italian and German display a fairly steady level of attention paid to the pandemic. 
However, the average rank of usage of the selected 1-grams slows down 
and starts to decay across many languages in April through the summer. 
In fact, the average rank of usage have dropped an order of magnitude in Indian, Russian, Korean, and Swedish.
While the number of new daily cases and deaths are climbing up again, 
we do not observe the same level of attention reciprocated on Twitter. 


\section{Concluding remarks}
\label{sec:covid19.concludingremarks}

We echo our main general observation of how COVID-19 has been discussed through
late April 2020:
\textbf{
After reacting strongly in late January to the news that a coronavirus-based disease
was spreading in China, attention across all but 2 of the 24 languages we survey dropped
through February before resurging in late February and through March.
}
We see abrupt shocks in time series as populations shifted rapidly to heightened
levels of awareness, particularly in the Italian time series.
In the time series for `virus', we see two and sometimes three peaks of attention
in the space of just a few months.
Our hope is that our collection of Twitter $n$-gram time series
that are especially relevant to April 2020
will be of benefit to other researchers.
The time series we share will, in part, reflect many other aspects beyond
mentions of `virus', which we have only briefly explored here.
\textbf{
Possible topics to investigate include
washing (including the soap and microbe emojis),
testing,
serology,
vaccine,
masks and protection equipment,
social and physical distancing,
terms of community support versus loneliness and isolation,
closures of schools and universities,
economic problems,
job loss,
and
food concerns.
}

We repeat that the lists we provide are meant to represent
the important $n$-grams of April 2020,
and we urge a degree of caution in the use of the data set.
As we have indicated above, our lists of $n$-grams contain some peculiarities
that will not be directly relevant to COVID-19.
Entertainment (e.g., movies, celebrities, and K-pop) and sports (football along with sports in the United States)
are standard fare on Twitter when no major events are taking place in the world.
The extent to which these aspects of Twitter
are submerged as pandemic related $n$-grams rise is of interest.

Finally, while we have been able to identify languages well,
geolocation is coarse and at best will be at the level of countries.
The strength of geolocation for our time series will
depend on the degree of localization of a given language
as well as Twitter user demographics.
We leave producing $n$-grams with serviceable physical location as
a separate project.
  

==> covid19-ngrams.highranks.tex <==
Retrieving English: 1gram -- 'virus'
Highest rank: 83.0 -- 2020-03-13
Retrieving Spanish: 1gram -- 'virus'
Highest rank: 96.0 -- 2020-03-14
Retrieving Portuguese: 1gram -- 'vírus'
Highest rank: 60.0 -- 2020-03-13
Retrieving Arabic: 1gram -- 'فيروس'
Highest rank: 119.0 -- 2020-03-16
Retrieving Korean: 1gram -- '바이러스'
Highest rank: 181.0 -- 2020-01-25
Retrieving French: 1gram -- 'virus'
Highest rank: 61.0 -- 2020-01-25
Retrieving Indonesian: 1gram -- 'virus'
Highest rank: 24.0 -- 2020-01-26
Retrieving Turkish: 1gram -- 'virüs'
Highest rank: 44.0 -- 2020-03-16
Retrieving German: 1gram -- 'Virus'
Highest rank: 201.0 -- 2020-03-14
Retrieving Italian: 1gram -- 'virus'
Highest rank: 61.0 -- 2020-02-24
Retrieving Russian: 1gram -- 'вирус'
Highest rank: 268.0 -- 2020-03-21
Retrieving Tagalog: 1gram -- 'virus'
Highest rank: 74.0 -- 2020-01-30
Retrieving Hindi: 1gram -- 'virus'
Highest rank: 921.5 -- 2020-03-04
Retrieving Persian: 1gram -- 'ویروس'
Highest rank: 39.0 -- 2020-03-22
Retrieving Urdu: 1gram -- 'وائرس'
Highest rank: 27.0 -- 2020-03-19
Retrieving Polish: 1gram -- 'wirus'
Highest rank: 149.0 -- 2020-03-11
Retrieving Catalan: 1gram -- 'virus'
Highest rank: 58.0 -- 2020-03-15
Retrieving Dutch: 1gram -- 'virus'
Highest rank: 170.5 -- 2020-03-17
Retrieving Tamil: 1gram -- 'virus'
Highest rank: 846.0 -- 2020-03-21
Retrieving Greek: 1gram -- 'ιός'
Highest rank: 206.0 -- 2020-03-10
Retrieving Swedish: 1gram -- 'virus'
Highest rank: 401.5 -- 2020-03-15
Retrieving Serbian: 1gram -- 'вирус'
Highest rank: 106.0 -- 2020-03-10
Retrieving Finnish: 1gram -- 'virus'
Highest rank: 224.5 -- 2020-03-19
Retrieving Ukrainian: 1gram -- 'вірус'
Highest rank: 134.0 -- 2020-03-22




Highest rank: 83.0 -- 2020-03-13
Retrieving Spanish: 1gram -- 'virus'
Highest rank: 96.0 -- 2020-03-14
Retrieving Portuguese: 1gram -- 'vírus'
Highest rank: 60.0 -- 2020-03-13
Retrieving Arabic: 1gram -- 'فيروس'
Highest rank: 119.0 -- 2020-03-16
Retrieving Korean: 1gram -- '바이러스'
Highest rank: 181.0 -- 2020-01-25
Retrieving French: 1gram -- 'virus'
Highest rank: 61.0 -- 2020-01-25
Retrieving Indonesian: 1gram -- 'virus'
Highest rank: 24.0 -- 2020-01-26
Retrieving Turkish: 1gram -- 'virüs'
Highest rank: 44.0 -- 2020-03-16
Retrieving German: 1gram -- 'Virus'
Highest rank: 201.0 -- 2020-03-14
Retrieving Italian: 1gram -- 'virus'
Highest rank: 61.0 -- 2020-02-24
Retrieving Russian: 1gram -- 'вирус'
Highest rank: 268.0 -- 2020-03-21
Retrieving Tagalog: 1gram -- 'virus'
Highest rank: 74.0 -- 2020-01-30
Retrieving Hindi: 1gram -- 'virus'
Highest rank: 921.5 -- 2020-03-04
Retrieving Persian: 1gram -- 'ویروس'
Highest rank: 39.0 -- 2020-03-22
Retrieving Urdu: 1gram -- 'وائرس'
Highest rank: 27.0 -- 2020-03-19
Retrieving Polish: 1gram -- 'wirus'
Highest rank: 149.0 -- 2020-03-11
Retrieving Catalan: 1gram -- 'virus'
Highest rank: 58.0 -- 2020-03-15
Retrieving Dutch: 1gram -- 'virus'
Highest rank: 170.5 -- 2020-03-17
Retrieving Tamil: 1gram -- 'virus'
Highest rank: 846.0 -- 2020-03-21
Retrieving Greek: 1gram -- 'ιός'
Highest rank: 206.0 -- 2020-03-10
Retrieving Swedish: 1gram -- 'virus'
Highest rank: 401.5 -- 2020-03-15
Retrieving Serbian: 1gram -- 'вирус'
Highest rank: 106.0 -- 2020-03-10
Retrieving Finnish: 1gram -- 'virus'
Highest rank: 224.5 -- 2020-03-19
Retrieving Ukrainian: 1gram -- 'вірус'
Highest rank: 134.0 -- 2020-03-22


==> covid19-ngrams.nutshell.tex <==
\todo{Write a 1--3 sentence nutshell (logline)}



==> covid19-ngrams.outtakes.tex <==
\begin{comment}
  
Iran, Coronavirus:

From: Nina Safavi Nina.Safavi@uvm.edu
Date: Thursday, March 26, 2020 at 4:39 PM
To: Aaron Schwartz Aaron.J.Schwartz@uvm.edu
Cc: "Jarlath P.M. O'Neil-Dunne" Jarlath.ONeil-Dunne@uvm.edu
Subject: Corona words

Hi Aaron,

I hope you and your family are doing well and staying safe. Attached are the corona related words and translations used in Iran. I’m including Jarlath here because he kindly approved part of my time to develop the list as a SAL service project.

I originally asked family members living in Iran to share common words that they noticed on social media describing the coronavirus pandemic. There wasn’t much of a response. Instead my mom added me to a 20 person family WhattsApp chat group that was all in Farsi and reflected their actual conversations. Tapping into my 2nd grade level Farsi reading ability, I could loosely follow and occasionally participate.  After a week, I exported the full text file and google translated everything. I added key words to your original list. She’s not a professional translator, but my mom double checked the translations and made some edits.

I’m not in regular communication with my family in Iran and this was a sweet and immersive experience. Their tone was generally positive, but concerned. They took every chance to make jokes and share stories/updates, while they are under quarantine. Luckily, no one in the circle was showing signs of corona. Some common themes were:
-Isolation during the week of the Iranian New Year (Nowrus)
-Sharing updates from Iranian government, and International sources like the WHO as well as non-authoritative sources.
-Iranians from northern regions of the country traveling to southern regions (Terhrani’s leaving the big city parallels what we’re seeing with New Yorkers in the US). Out-of-towners are identified by their license plates.
-Everyone in the group was staying inside. All non-essential businesses/offices are closed.
-Many believe the virus spread from the holy City of Qom where there was a group of Chinese visitors.
-There were mild concerns of other disasters coming, such as new deadlier viruses (new strand of corona, hanta virus), and projection of heavy rain and flooding.
-The Iranian government is going to give everyone financial relief funds.
-Mostly the conversations were familiar and involved what meals were being cooked up, sending well wishes, sharing jokes/funny memes.
-No hashtags were used, but that’s as expected on WhattsApp

I hope this is helpful. Let me know if I can help in any other way.

Take care,
Nina

\end{comment}

\begin{comment}
  

Indonesia is really in bad shape. So initially, around January and February, the government focussed on economic issues and the evacuation of Indonesians from Wuhan and cruise ships.

The health minister is notoriously an incompetent military doctor. He downplayed the virus and tell people to “enjoy”. Things started to change when a cabinet member (transportation minister) tested positive.

I believe Indonesia is really undertested, the official numbers for today are 790 positives and 58 deaths. they are mostly in Greater Jakarta area
There’re stay-at-home suggestions from central and local governments. Unfortunately, during this period many people chose to returned to their hometowns and hence spread the virus.

April would be important for Indonesia

In terms of public opinion, I think, there are two polarized groups. Say 20% of population who want stringent lock down policy and 80% of middle lower income groups who depend on daily wages. So there’s the tension between health and economic considerations.
That’s why the government chose not to enforce lock down because of the potential social political backlash.
The government’s plan is to have testing as many and fast as possible. Although, it’s still not clear how to do that and whether we have the necessary resources

Roby  2:04 AM
My affiliation
Roby Muhamad
International Class Program
Faculty of Social and Political Sciences
University of Indonesia

Roby  5:12 AM
103 new cases, so total as of today is 893 positives
20 new death, total 78 deaths
\end{comment}



The increase in the total use of the emoji {\NotoEmoji\symbol{"1F9A0}}




\begin{table*}
  \begin{tabular}{rrr}
    English &
    Italian & 
    Spanish \\
    \begin{tabular}{r}
      virus \\
      quarantena \\
      contagio \\
      intensiva \\
      medici \\
      2020 \\
      terapia \\
      mascherine \\
      <U+1F97A> \\
      misure \\
      ospedali \\
      . \\
      emergenza \\
      infermieri \\
      Lombardia \\
      , \\
      sanitaria \\
      corona \\
      l'emergenza \\
      sanità \\
      mascherina \\
      @RobertoBurioni \\
      situazione \\
      sanitario \\
      Licia \\
      chiuse \\
      positivo \\
      isolamento \\
      casi \\
      positivi \\
      casa \\
      l’emergenza \\
      <U+1F921> \\
      Patrick 
    \end{tabular}
    &
    \begin{tabular}{r}
      virus \\
      quarantena \\
      contagio \\
      intensiva \\
      medici \\
      2020 \\
      terapia \\
      mascherine \\
      <U+1F97A> \\
      misure \\
      ospedali \\
      . \\
      emergenza \\
      infermieri \\
      Lombardia \\
      , \\
      sanitaria \\
      corona \\
      l'emergenza \\
      sanità \\
      mascherina \\
      @RobertoBurioni \\
      situazione \\
      sanitario \\
      Licia \\
      chiuse \\
      positivo \\
      isolamento \\
      casi \\
      positivi \\
      casa \\
      l’emergenza \\
      <U+1F921> \\
      Patrick 
    \end{tabular}
    &
    \begin{tabular}{r}
      virus \\
      quarantena \\
      contagio \\
      intensiva \\
      medici \\
      2020 \\
      terapia \\
      mascherine \\
      <U+1F97A> \\
      misure \\
      ospedali \\
      . \\
      emergenza \\
      infermieri \\
      Lombardia \\
      , \\
      sanitaria \\
      corona \\
      l'emergenza \\
      sanità \\
      mascherina \\
      @RobertoBurioni \\
      situazione \\
      sanitario \\
      Licia \\
      chiuse \\
      positivo \\
      isolamento \\
      casi \\
      positivi \\
      casa \\
      l’emergenza \\
      <U+1F921> \\
      Patrick 
    \end{tabular}
    \\
  \end{tabular}
  \caption{
    The 25 languages for which we provide Covid-19 related time series.
    Building on 
  }
  \label{tab.covid19.topwords}
\end{table*}


\includegraphics[height=1em]{microbe_1f9a0.png}
\includegraphics[height=1em]{face-with-pleading-eyes_1f97a.png}


Google: 
{\NotoEmoji
\symbol{"1F97A}%
\symbol{"1F637}%
\symbol{"1F451}% 
\symbol{"1F9A0}%
\symbol{"1F9FC}%
\symbol{"1F590}%
\symbol{"1F927}%
\symbol{"1F3E5}% 
\symbol{"1F691}%
}




Twitter:
{\TwemojiMozilla
\symbol{"1F97A}%
\symbol{"1F637}%
\symbol{"1F451}% 
\symbol{"1F9A0}%
\symbol{"1F9FC}%
\symbol{"1F590}%
\symbol{"1F927}%
\symbol{"1F3E5}% 
\symbol{"1F691}%
}

{
  \NotoSansCJKkr
  바이러스
}

We have recently processed this corpus of tweets to identify and extract day-scale
Zipf distributions
for 1-, 2-, and 3-grams along with
day-scale $n$-gram time series for over 150 languages~\cite{alshaabi2020a}.


Nicholas Danforth

  “Turkish is always funny on these things because you’ll get all the different variations of a word showing up separately. like “refugees” “refugee” “the refugees” “with the refugees” etc. the words themselves all sound about right. Im always intrigued by what “skin color” people in different countries use for their emojis.”
:+1:


danforth  10:49 AM
From a friend that speaks Swedish: “I am curious how the verb `to close’ is on that list four times in the top 80, yet much of Sweden remains open - including elementary and middle schools. Also hands is 31 but wash doesn’t appear until 83 :joy:”


==> covid19-ngrams.pacs.tex <==
\pacs{89.65.-s,89.75.Da,89.75.Fb,89.75.-k}

%% 89.65.-s	Social and economic systems
%% 89.75.Da	Systems obeying scaling laws
%% 89.75.Fb	Structures and organization in complex systems
%% 89.75.-k	Complex systems (for complex chemical systems, see 82.40.Qt; for biological complexity, see 87.18.-h)



==> covid19-ngrams.settings.tex <==
\lefthyphenmin=3
\righthyphenmin=2

\def\topfraction{1.0}

%% make tables and figures be of the same type
%% https://tex.stackexchange.com/questions/127742/place-floating-tables-and-figures-in-order-of-appearance
\makeatletter
\let\ftype@table\ftype@figure
\makeatother

%% \usepackage{fontawesome} 
%% \usepackage{fontspec} 
%% \newfontfamily{\NotoEmoji}{NotoColorEmoji.ttf}[Renderer=Harfbuzz]
%% \newfontfamily{\TwemojiMozilla}{TwemojiMozilla.ttf}[Renderer=Harfbuzz]
%% \newfontfamily{\SymbolaEmoji}{Symbola.ttf}[Renderer=Harfbuzz]
%% \newfontfamily{\NotoSansCJKkr}{NotoSansCJKkr.otf}[Renderer=Harfbuzz]

%% for figure adjustment
%% https://tex.stackexchange.com/questions/91566/syntax-similar-to-centering-for-right-and-left
%% \usepackage[export]{adjustbox}

%% helpful for complicated papers
%% in finding out which figures, etc. are not being referenced

%% \usepackage{refcheck}
%% also helpful, highlighting the value of adding taxonomy to labels:
%% grep -A 1 refcheck paper-template-revtex4.log | grep -A 1 fig:

%% url style:
\urlstyle{same}

%% build papers out of todo lists
\usepackage{color}
\newcommand{\todo}[1]{\noindent\textcolor{blue}{{$\Box$ #1}}}

\usepackage{graphicx,epsfig,verbatim,enumerate}
\usepackage{amssymb,amsmath}
\usepackage{ifthen}

\usepackage{longtable}

\usepackage{mathtools}
%% \usepackage{abraces}

%% \usepackage{tikz-cd}
%% \usetikzlibrary{arrows}
%% \tikzset{
%%   commutative diagrams/.cd,
%%   arrow style=tikz,
%%  diagrams={>=space}}

\newboolean{twocolswitch}

\newcommand{\avg}[1]{\left\langle#1\right\rangle}
\newcommand{\tavg}[1]{\langle#1\rangle}

\newcommand{\LavgHa}[2]{\tavg{L_{#1,#2}}}
\newcommand{\LavgHaN}[2]{\tavg{L_{#1,#2}}}
\newcommand{\Lavg}{\tavg{L}}

\newcommand{\sindex}[1]{}
\newcommand{\nindex}[1]{}

\newcommand{\etal}{\textit{et al.}}
\newcommand{\www}[1]{\url{#1}}
\newcommand{\req}[1]{(\ref{#1})}
\newcommand{\Req}[1]{Eq.~(\ref{#1})}

% lettrines
\usepackage{lettrine}

\newcommand{\tbf}{\textbf}
\newcommand{\tit}{\textit}

%% differential equations and integrals
\newcommand{\dee}[1]{\textnormal{d}#1}
\newcommand{\pdiff}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pdiffsq}[2]{\frac{\partial^2 #1}{{\partial #2}^2}}
\newcommand{\diff}[2]{\frac{{\rm d}#1}{{\rm d}#2}}
\newcommand{\diffsq}[2]{\frac{{\rm d}^{2}#1}{{\rm d} {#2}^2}}
\newcommand{\tdiff}[2]{\textnormal{d} #1/\textnormal{d} #2}
\newcommand{\tdiffsq}[2]{\textnormal{d}^{2} #1/\textnormal{d} {#2}^2}
\newcommand{\tpdiff}[2]{\partial #1/\partial #2}
\newcommand{\tpdiffsq}[2]{\partial^2 #1/\partial {#2}^2}
\newcommand{\postdee}[1]{\,\textnormal{d}#1}


\newcommand{\Prob}[1]{{\rm Pr}\left(#1\right)}

%% contagion

% \newcommand{\kstar}{d^{\ast}}
% \newcommand{\kstari}{k_i^\ast}
\newcommand{\kstar}{d^\ast}
\newcommand{\kstari}{d_i^\ast}

\newcommand{\dstar}{d^\ast}
\newcommand{\dstari}{d_i^\ast}

\newcommand{\phifix}{{\phi^{\ast}}}
\newcommand{\phifixc}{{\phi_c^{\ast}}}
\newcommand{\phifixb}{{\phi_b^{\ast}}}

\newcommand{\phiiactive}{\phi_{i,t}}

\newcommand{\phiiup}{{\phi_{i,\rm on}}}
\newcommand{\phiidown}{{\phi_{i,\rm off}}}

\newcommand{\phiup}{{\phi_{\rm on}}}
\newcommand{\phidown}{{\phi_{\rm off}}}


\newcommand{\Gfun}{G}

\newcommand{\dstardist}{g}
\newcommand{\dosedist}{f}
\newcommand{\dosedistk}{f^{k\star}}

% chaotic contagion
\newcommand{\edgeinfprob}{\rho}
\newcommand{\nodeinfprob}{\phi}

\newcommand{\avgdegree}{k_{\rm avg}}

\newcommand{\stateA}{S_{0}}
\newcommand{\stateB}{S_{1}}

\newcommand{\lcce}{H}

%% \newcommand{\effectivecount}{f_{\textnormal{eff}}}

\newcommand{\effectivecount}{f_{q,\textnormal{exp}}}
\newcommand{\effectivecountq}[1]{f_{#1,\textnormal{exp}}}

\newcommand{\simonrho}{\rho}
\newcommand{\zipfexponent}{\alpha}

\newcommand{\partitionprob}{q}
\newcommand{\partitiontype}[1]{$\partitionprob$$=$$#1$}

\newcommand{\onehalf}{\frac{1}{2}}
\newcommand{\onequarter}{\frac{1}{4}}

\newcommand{\clgamma}{\hat{\zipfexponent}}
\newcommand{\xmin}{r_{\textnormal{max}}}
\newcommand{\kstat}{D}
\newcommand{\clp}{\textnormal{$p$-value}}
\newcommand{\sigamma}{1-\simonrho}




==> covid19-ngrams.title.tex <==
How the world's collective attention is being paid to a pandemic:\\
COVID-19 related $n$-gram time series for 24 languages on Twitter

%% Measuring the world's collective attention being paid to a pandemic

%% How the world's collective attention is being paid to a pandemic: COVID-19 related 1-gram time series for 24 languages on Twitter

